Multi-Higgs Models: model building, phenomenology and renormalization

In this thesis, we investigate several aspects of models with a multiplicity of Higgs bosons. We start by focusing on models with two Higgs doublets. We claim that one of the most used models in the literature -- the so-called real 2-Higgs-Doublet Model (2HDM) -- is inconsistent. We give special emphasis to the model that corrects it in the most simple way, the complex 2HDM; we study its phenomenology in the lowest order of perturbation theory and describe its renormalization in the following order. Motivated by this renormalization, we analyze in detail tadpole schemes that allow the selection of the true vacuum expectation value in models with spontaneous symmetry breaking, and we propose a theorem regarding the finitude of Green's functions with corrections to the external legs. Given the complexity of the calculations involved, it is crucial to dispose of an appropriate software. We therefore present FeynMaster, which calculates, among other things, Feynman rules, radiative corrections and counterterms in a simultaneously automatic and flexible way. We use the potential of FeynMaster to investigate two new projects related to multiple scalar bosons: first, we consider the class of models with a generic number of scalar doublets and singlets, and investigate radiative corrections to the $Z \to b \bar{b}$ process in this context; then, we explore the phenomenology of a model based on the linear seesaw hypothesis, which, in addition to two scalar doublets, includes a complex singlet.

==> Inputs/Biblio.tex <==
\begin{thebibliography}{199} 
	
	%\cite{Fontes:2014tga}
	\bibitem{Fontes:2014tga}
	D.~Fontes, J.~C.~Romão and J.~P.~Silva,
	%``A reappraisal of the wrong-sign $hb\overline{b}$ coupling and the study of $h \rightarrow Z \gamma$,''
	Phys.\ Rev.\ D {\bf 90} (2014) 015021
	[arXiv:1406.6080 [hep-ph]].
	%%CITATION = ARXIV:1406.6080;%%
	%2 citations counted in INSPIRE as of 24 Aug 2014
	
\end{thebibliography}


==> Inputs/Bolsa.tex <==
\cleardoublepage

{\FontT
\null\vfill

\begin{flushright}
\begin{minipage}{0.75\textwidth}
\begin{flushright}
Este trabalho foi financiado pela Fundação para a Ciência e Tecnologia\\
(FCT), sob os contratos 
UID/FIS/00777/2013 e SFRH/BD/135698/2018.
\end{flushright}
\end{minipage}\\[10mm]

\begin{minipage}{0.9\textwidth}
\begin{flushright}
This work has been financially supported by \textit{Fundação para a Ciência}\\
\textit{e Tecnologia} (FCT), under the grants
UID/FIS/00777/2013 and SFRH/BD/135698/2018.
\end{flushright}
\end{minipage}


\end{flushright}
}

\cleardoublepage


==> Inputs/Cover-draft.tex <==
% ====================================== Page numbering
\thispagestyle {empty}

% ====================================== Font Sizes
\def\FontLL{% 18 pt normal
  \usefont{T1}{cmr}{m}{n}\fontsize{18pt}{18pt}\selectfont}
\def\FontL{% 16 pt normal
  \usefont{T1}{cmr}{m}{n}\fontsize{17.28pt}{16pt}\selectfont}
% \usefont{T1}{pvh}{m}{n}\fontsize{16pt}{16pt}\selectfont}
\def\FontM{% 14 pt normal
  \usefont{T1}{cmr}{m}{n}\fontsize{14pt}{14pt}\selectfont}
% \usefont{T1}{phv}{m}{n}\fontsize{14pt}{14pt}\selectfont}
\def\FontS{% 12 pt normal
  \usefont{T1}{cmr}{m}{n}\fontsize{12pt}{12pt}\selectfont}
% \usefont{T1}{phv}{m}{n}\fontsize{12pt}{12pt}\selectfont}
\def\FontT{% 10 pt normal
  \fontsize{10pt}{10pt}\selectfont}


% ====================================== Logo
\noindent \includegraphics[width=5cm]{ist_logo.jpg}


% ====================================== Cover information
\begin{center}

%\vspace{3cm}

{\FontL \textbf{UNIVERSIDADE DE LISBOA}} \\
{\FontL \textbf{INSTITUTO SUPERIOR TÉCNICO}} \\

%\vspace{10mm}
\vspace{15mm}

{\FontLL \textbf{Multi-Higgs Models:}} \\
{\FontM \textbf{model building, phenomenology and renormalization}} \\

%\vspace{10mm}
\vspace{15mm}

{\FontM \textbf{Duarte Sarmento de Sousa Machado Fontes}} \\
\end{center}

%\vspace{5mm}
\vspace{10mm}

{\FontS \textbf{Supervisor}: Doctor Jo\~{a}o Paulo Ferreira da Silva} \\
{\FontS \textbf{Co-Supervisor}: Doctor Jorge Manuel Rodrigues Crispim Rom\~{a}o}

\begin{center}

%\vspace{5mm}
\vspace{10mm}

{\FontS \textbf{Thesis specifically prepared to obtain the PhD Degree in}} \\[2mm]
{\FontL \textbf{Physics}}


\vspace{35mm}
{\FontL \textbf{Draft}}

%\vspace{10mm}

%{\FontS \textbf{Jury}}
%\end{center}
%
%\vspace{-2mm}
%
%{\FontS \textbf{Chairperson}: \\
%%
%\hphantom{\hspace{6.5mm}} Prof. Dr. M\'{a}rio Jo\~{a}o Martins Pimenta, Instituto Superior Técnico (IST), Universi-\\
%\hphantom{\hspace{25mm}} dade de Lisboa (UL)} 
%
%\vspace{2mm}
%
%{\FontS \textbf{Members of the Commitee}:
%
%\begin{addmargin}[8mm]{0mm}
%Prof. Dr. Ansgar Denner, Universität Würzburg \\
%%
%Prof. Dr. Rui Alberto Serra Ribeiro dos Santos, Instituto Superior de Engenharia \\
%%
%\hphantom{\hspace{17mm}} de Lisboa, Instituto Politécnico de Lisboa \\
%%
%Prof. Dr. José Guilherme Milhano, IST, UL \\
%%
%Prof. Dr. Jorge Manuel Rodrigues Crispim Rom\~{a}o, IST, UL
%\end{addmargin}
%}

\vspace{5mm}

%\begin{center}
%{\FontS \textbf{Funding}\\
%Grants UID/FIS/00777/2013 and SFRH/BD/135698/2018 from Fundação para a Ciência e Tecnologia (FCT).
%}



\vfill


{\FontM \textbf{June 2021}}

\end{center}

\pagebreak
\thispagestyle {empty}
\cleardoublepage




==> Inputs/Dedication.tex <==
\cleardoublepage

{\FontT
\null\vskip 3cm

\begin{flushright}
\begin{minipage}{0.75\textwidth}
\begin{flushright}
Dedicado à minha mãe
\end{flushright}
\end{minipage}


\end{flushright}
}

\cleardoublepage

